Reducing Access Disparities in Networks using Edge Augmentation

In social networks, a node's position is a form of \it{social capital}. Better-positioned members not only benefit from (faster) access to diverse information, but innately have more potential influence on information spread. Structural biases often arise from network formation, and can lead to significant disparities in information access based on position. Further, processes such as link recommendation can exacerbate this inequality by relying on network structure to augment connectivity. We argue that one can understand and quantify this social capital through the lens of information flow in the network. We consider the setting where all nodes may be sources of distinct information, and a node's (dis)advantage deems its ability to access all information available on the network. We introduce three new measures of advantage (broadcast, influence, and control), which are quantified in terms of position in the network using \it{access signatures} -- vectors that represent a node's ability to share information. We then consider the problem of improving equity by making interventions to increase the access of the least-advantaged nodes. We argue that edge augmentation is most appropriate for mitigating bias in the network structure, and frame a budgeted intervention problem for maximizing minimum pairwise access. Finally, we propose heuristic strategies for selecting edge augmentations and empirically evaluate their performance on a corpus of real-world social networks. We demonstrate that a small number of interventions significantly increase the broadcast measure of access for the least-advantaged nodes (over 5 times more than random), and also improve the minimum influence. Additional analysis shows that these interventions can also dramatically shrink the gap in advantage between nodes (over \%82) and reduce disparities between their access signatures.

==> definitions_cp.tex <==
\section{Access-based Definitions}
\label{sec:definitions}
Since our problem is in information access setting and not in graph theory, it is justifiable to redefine some graph theoretical terms in the new setting. We show that these measures are not the same as their graph theoretical equivalence, and they better capture the concepts such as distance, diameter, and betweenness centrality in information access setting.

\paragraph{Access Distance} For nodes $v_i$ and $v_j$ in the network, the access probability $p_{ij}$ can be described as the \emph{access distance} of $v_i$ to $v_j$. In opposed to the graph theory definition, where the distance of node $v_i$ to $v_j$ is defined as the number of the edges in the shortest path connecting $v_i$ to $v_j$, in our setting, the distance (or access distance) is defined as the ratio of IC instances where node $v_i$ is connected to node $v_j$. In other words, the probability of access of node $v_i$ to information from node $v_j$. Note that these two definitions are not the same. For example in Figure~\ref{fig:distance}, the distance of node $a$ to $b$ is $1$, meaning it has a smaller distance than node $c$ to $d$ with distance of $2$. Although in the IC model the distance of $a$ to $b$ is $\alpha$, while the access of $c$ to $d$ is $(1 - \alpha^{2})^t$. For values of $t > \frac{\log(1 - \alpha)}{\log(1 - \alpha^2)}$, the access of $c$ to $d$ is higher than the access of $a$ to $b$. By selecting the information spread model, we redefine the distance between nodes based on the model selected (in our case IC model).%Similarly, Jalali et al.~\cite{jalali2020unfairness} computed the distance between nodes as their access, although they used a different model for modeling information spread.

\begin{figure}
\centering
\tikzstyle{vertex}=[circle,fill=black,minimum size=5pt,inner sep=2pt]
\tikzstyle{circled} = [draw, blue, thick, circle, minimum size=.55cm]
\tikzstyle{edge}=[<-,color=black,line width=1.5]
\tikzstyle{edgeback}=[->,color=black,line width=1.5]
\tikzstyle{edgelabel}=[color=black]
\begin{tikzpicture}[scale=0.8, auto]

        \node[vertex] (a) at (-3,0) [label=below:$a$]{};
	\node[vertex] (b) at (-1,0) [label=below:$b$]{}
		edge[color=black,line width=1.5] node {} (a);

	\node[vertex] (c) at (3,1) [label=below:$c$]{};
	\node[vertex] (d) at (3,-1) [label=below:$d$]{};
	\node[vertex] (v1) at (1,0) [label=below:$v_1$]{}
		edge[color=black,line width=1.5] node {} (c)
		edge[color=black,line width=1.5] node {} (d);
	\node[vertex] (v2) at (2,0) [label=below:$v_2$]{}
		edge[color=black,line width=1.5] node {} (c)
		edge[color=black,line width=1.5] node {} (d);
	\node[draw=none] at (3,0) {$\cdots$};
	\node[draw=none] at (4,0) {$\cdots$};
	\node[vertex] (vn) at (5,0) [label=below:$v_t$]{}
		edge[color=black,line width=1.5] node {} (c)
		edge[color=black,line width=1.5] node {} (d);

\end{tikzpicture}
\caption{One the left: nodes with one path of length $1$ connecting them. On the right: nodes with $n$ paths of length $2$ connecting them.}
\label{fig:distance}
\end{figure}

\begin{defn}[Access Distance] We define access distance of node $v_i$ to node $v_j$ as the the probability of $v_i$ receiving the information from node $v_j$.
\[ \text{\dist{}} (i, j) = p_{ij} \]
\end{defn}

\paragraph{Access Diameter} The node-to-node distances are often studied in terms of the diameter described as the length of the shortest path. The access diameter refers to nodes that have the worst-case cost of routing a point-to-point message. Although in the information access scenario, the diameter of the network would translate into maximum access distance among nodes. Similarly we can define the \emph{access diameter} as:

\begin{defn}[Access Diameter] The access diameter of network $G$ is defined as the maximum access distance between any pair of nodes.

\[ \text{\diam{}}_{G} = \max_{v_i \neq v_j \in V} p_{ij} \]
\end{defn}

Consequently, any diameter-defining node (with distance $\text{\diam{}}_{G}$ to some other node) would be defined as \emph{peripheral node}. Furthermore, in the same way, the node with minimum maximum distance from all other nodes would be the \emph{central node}.

\paragraph{Access Centrality} Betweenness centrality is a way of detecting the amount of influence a node has over the flow of information in a graph. It is often used to find nodes that serve as a bridge from one part of a graph to another. In graph theory, betweenness centrality is a measure of centrality in a graph based on shortest paths. For every pair of nodes in a connected graph, there exists at least one shortest path between the nodes. The betweenness centrality for each node is the proportion of these shortest paths that pass through the node.

\[ g(c) = \sum_{v_i \neq v_j \neq v_c \in V} \frac{\sigma_{ij}(c)}{\sigma_{ij}} \]

In our setting we can define a similar measure based on centrality called \ctradv{}, to measure the brokerage ability of a node to act as a bridge, connecting different parts of the network to each other. Although instead of computing the proportion of shortest paths that pass through a node, we measure the proportion of IC instances that pass through a node. For every pair of nodes in the network, we compute the proportion of IC instances that pass through this node. This mean how much this node is used for communication (transferring information) by other nodes. The average over this measure for all pairs in the network, would give us the overall \ctradv{} of the node.

For computing the \ctradv{} of node $v_c$ over each pair, we need to remove $v_c$, and rerun the simulation to estimate the access between the pair in absence of $v_c$ ($p_{ij} (\cancel{c})$). This is the amount of access that "does not" pass through $v_c$. Subtracting it from their access before the intervention (removal of $v_c$), and we have the amount of access that passes through $v_c$ as $p_{ij} (c) = p_{ij} - p_{ij} (\cancel{c})$.

\begin{defn}[Access Centrality] We define the access centrality of node $v_c$ as\footnote{To normalize this values, we can divide them by ${n-1} \choose 2$.}:
\[\text{\cent{}} (c) = \sum_{v_i \neq v_j \neq v_c \in V} \frac{p_{ij} (c)}{p_{ij}} \]
\end{defn}

To help understand the measure, consider an open triad. The middle node can act as a broker, moving information from one side to the other side. The broker node has complete \ctradv{} over the other two nodes, meaning that every information passing from one node to the other should pass through the broker node, and the broker node has the ability to influence the other two without them having access to each other. So, the broker node has \ctradv{} value of $1$ over the other two, and the other two have \ctradv{} value of $0$.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

==> edge_cp.tex <==
\section{Proposing Edge Intervention}
\label{sec:edge}

\abnote{When to present Proposing Edge Interventions section: 1) after Background, since it can be considered as the motivation of the paper. It also explains why we are jumping from Influence Maximization problem to a new problem. The material would also be required before introducing the advantage measures. But the problem here is that this section is dividing the two definition sections (Background and Access-based Definitions). 2) before Maximizing the Minimum Access, since it is part of the problem definition. 3) Best alternative would be after Access-based Definitions. This will resolve all the problems mentioned in (1), except the one mentioned in (2).}
In influence maximization started with the purpose of maximizing the spread of innovation with respect to a single source / piece of information. Later, the problem has been adopted to applications in public health awareness. However, we argue that access to all information and all individuals is important and not just one. It no longer makes sense to focus on interventions that sources spread specific information in this new setting. Instead, the natural intervention is to add an edge. These edge-based interventions represent the idea of adding purposefully selected weak ties to the network. Unlike node interventions, they are capable of mitigating the bias in the structure of the network and increasing the overall connectivity of the network. In particular we provide three reasons why edge interventions are preferred:

\paragraph{Variety} Ideas come over a variety of paths from a variety of sources~\cite{von1988sources, geroski2002learning, menon2003valuing}, and access to a broader diversity of information and a larger number of individuals is important~\cite{granovetter77strength}, providing a vision advantage that can translate into social capital~\cite{burt2004holes}. For example in networks such as LinkedIn, at every moment important information are being announced from different sources. However, in the influence maximization setting, there is a single source of information, and additional seeds are selected to spread the information from this source. We argue that there are various sources of information in the network, and even each person can be considered as a potential source of information, each spreading their unique piece of information. Not only these sources may be unknown to us, but also they may change over time. It is not plausible anymore to find these sources and select additional seeds to spread their information as in the influence maximization setting.
	% Individuals are usually aware of opportunities in their social circle. In online social networks, important information comes not from one source but various sources. Adam Smith noted that "when the mind is employed about a variety of objects it is somehow expanded and enlarged~\cite{smiths1766}."
	% For example, in job hiring networks, it may be beneficial to connect nodes to a specific node that frequently announces job openings. Although next time there may be another job opening from a different source. We can not decide which nodes are important and which ones are not. It is premature to increase the connectivity of all nodes only to a selected set of nodes in the network.
	
\paragraph{Structure} Granovetter~\cite{granovetter77strength} introduced the idea of network manipulation to achieve specific goals. Since network structure can represent a form of social capital, and our underlying problem here is the bias in the network structure, the kind of interventions that make sense here is structural interventions that are more naturally caused as edge interventions. It is not just which recruiter reaches out to the user that determines her access to job information, but also her connection to friends and family members who pass on information. This new setting represents the idea of adding selected weak ties into the social network. Moreover, weak ties are more effective in the diffusion of ideas, influence, and information. Weak ties increase flow by creating more and shorter paths. Information diffused can reach many people and traverse greater social distance when passed through weak ties rather than strong ones.
	
\paragraph{Voice} Influence maximization setting promotes one type of information from a single source. Node interventions increases the reach of the already advantaged nodes. Reach like access is another form of advantage~\cite{granovetter77strength}. The influence of an individual is correlated with their reach to other members, and node interventions give more advantage to these selected individuals~\cite{jackson19human}. Instead of only increasing the access to some specific nodes, we argue that each person has the right to be heard by others. As in edge intervention setting which increases the overall connectivity of the graph, and reach of every node, and not only a few advantaged nodes.

==> np_proof.tex <==
\section{Maximizing the Minimum Access (or Multi-Signal Edge Max-Min)}
\label{sec:max-min}

\abnote{include in the support that max-min is sufficient for maximizing other measures of advantage.}
In this section we use a normative framework to decide which advantage measure should we choose to base the optimization the problem on. We present argument for preventing the rich from getting riche. Then based on the Rawlsian maximin argument we propose maximizing the advantage of the least advantaged.

One of the promises of a highly connected world is an impartial spread of opinions driven by free and unbiased sources of information leading to an equitable exposure of opinion to the wide public. On the contrary, the social network platforms that are currently governing news diffusion, while offering many seemingly-desired features like searching, personalization, and recommendation, are reinforcing the centralization of information spreading and the creation of what is often termed echo chambers and filter bubbles~\cite{Becker2020}.

%\subsection{Choice of Advantage Notion (Normative framework):}
%\label{sec:measure-choice}
Although, optimizing based on the \aveadv{} measure may encourage interventions connecting the poor nodes to well-positioned nodes. If one wants information, it makes sense to connect with someone well-positioned in the network. Therefore, someone who has more connections becomes more attractive to connect to~\cite{jackson19human}, which leads to a rich-get-richer phenomenon and increases the power of the rich even more~\cite{burt1999opinion}. Link recommendation algorithms are already using this approach by suggesting users with high visibility.

On the other hand, optimization based on \minadv{} measures may avoid the rich get richer pitfall by encouraging the connection of most disadvantaged nodes. As John Stuarts Mill's noted, "it is hardly possible to overrate the value . . . of placing humans in beings in contact with persons dissimilar to themselves and with modes of thought and action unlike those with which are familiar . . . Such communication has always been and is peculiarly in the present age, one of the primary sources of progress~\cite{miller1848}."

%There have been lots of work on polarization, and attempts on mitigating the phenomenon. By increasing the similarity of access of nodes, they would have similar exposure to different news and ideas. Hence this approach also mitigates the concept of polarization in social networks.

%\subsection{Problem Statement}
Rawl claims that persons should act according to \emph{Maximin Principle}: Maximizing the welfare of the worst-off person. Following the Rawlsian theory~\cite{rawls2009theory}, our goal is to maximize the advantage of the most disadvantaged. Then the problem turns into minimizing the access diameter of $G$ or in other words minimizing the maximum access distance between nodes in $G$.

Here we provide other normative reasons to pick the \minadv{} measure as the representation of the advantage of a node:
\begin{itemize}
	\item Minorities may have common interests but not enough influence to accomplish them. This approach of connecting small groups will oppose the ever-increasing power of central and influential nodes.
	\item Minorities would have a chance to support each other, increase their influence, and access important information. The idea of connecting minorities has been working. Considering the LGBTQ community, each group separately may not have enough voice and influence to fight for their rights, but connecting them would increase their power and give them an independent voice to achieve their goals. As an evidence Kogan et al. show that geographically vulnerable (disadvantaged) propagate more information during the disaster period, and are more likely to propagate tweets from other geographically vulnerable users, especially during a disaster\cite{Kogan2015Think}.
	\item One fundamental parameter of networks that many people are interested in is the distance between pairs of nodes. Minimizing the diameter of the network can speed up communication in a network~\cite{demaine2010diam}. It can also bring all nodes closer to a common information access profile.
\end{itemize}

\begin{defn}
The overall welfare of a graph $G=(V,E)$ is 
\[\mu_G(E) = \min_{v_i \in V} \text{\minadv{}}(v_i) = \min_{v_i , v_j \in V} \text{\dist{}}(v_i, v_j)\]
 \end{defn}

Our primary goal in the study of information flow is to find a \emph{budgeted intervention}: a set of edges $E^+$ of size $k$ for a given graph $G$ with maximum welfare
\[E^* = \argmax_{\substack{E^+ \cup E:\\|E^+ | \le k}}\mu_G(E^+ \cup E)\]
In other words, $E^*$ is the initial edges $E$ along with a set of $k$ edges which maximizes welfare for $G$.

\abnote{Lemma here!}
The access between nodes is dependent on the paths connecting them. Although computing access is $\#p-hard$~\cite{}, there are a few rules that can help us in the proof. The first rule is that the access from $v_i$ to $v_j$ is at least $\alpha$ to the power of the length of any path from $v_i$ to $v_j$. The second important rule is the access from $v_i$ to $v_j$ increases if and only if that a path/route is added from $v_i$ to $v_j$.

\begin{defn}[Multi-Signal Edge Max-Min] Given a graph $G = (V, E)$ and a welfare function $\mu_{G}(E) = \min_{v_i , v_j \in V} p_{i,j}$, find an intervention $E^*$ of size $k$ that maximizes $\mu_{G} (E \cup E^*)$.
\end{defn}

\begin{theorem}\label{thm:multi_edge_maxmin_hardness}
Suppose $\alpha < \frac{\sqrt{5}-1}{2}$. Then \emph{Multi-Signal Edge Max-Min} is NP-hard, and cannot be approximated better than $\mathcal{O}(\alpha)$ and if furthermore $\alpha = \mathcal{O}(1/n)$ then the maximum cannot be attained efficiently without an additional $\mathcal{O}(\ln n)$ factor interventions.
\end{theorem}

\begin{proof}
We reduce from {\sc Set Cover}, where an instance is defined by a collection of subsets $S = {S_1,\ldots, S_m}$ over a ground set $X = \{x_1,\ldots,x_n\}$ and an integer $k$, and the decision problem is whether or not there is a collection of $k$ subsets whose union is $U$.  Further, we can assume $k < n < m$. Given such an instance, we construct a directed graph (example showed in Figure~\ref{fig:np_hardness}). We start with the natural directed bipartite graph corresponding to a set cover instance, where there is a vertex $S_i$ corresponding with each set $S_i$ and a vertex $x_j$ corresponding with each element $x_j$.  There is a directed edge from $S_i$ to $x_j$ whenever $x_j$ is contained in $S_i$. We then add two extra vertices $u$ and $v$. We add a directed edges, one from $u$ to $v$ and from each vertex $x_j$ corresponding with one of the elements to $u$. We also add edges from $v$ to each vertex $S_i$ corresponding with one of the sets and also in the reverse direction. We ask to maximize the minimum pairwise probability by adding $k$ edges.

\begin{figure}
\centering
\tikzstyle{vertex}=[circle,fill=black,minimum size=5pt,inner sep=2pt]
\tikzstyle{circled} = [draw, blue, thick, circle, minimum size=.25cm]
\tikzstyle{edge}=[<-,color=black,line width=1.5]
\tikzstyle{edgeback}=[->,color=black,line width=1.5]
\tikzstyle{edgelabel}=[color=black]
\begin{tikzpicture}[scale=0.8, auto]

 %\node[vertex] (u) at (0,1) [label=left:$u$]{};
 \node[vertex] (v) at (0,0) [label=above:$v$]{};

 \node[vertex] () at (-1,-1){};
 \node[vertex] (s1) at (-1,-1) [label=left:$S_1$]{}
 	edge[edge] node {} (v);
 \node[vertex] (s2) at (0,-1) [label=right:$S_2$]{}
 	edge[edge] node {} (v);
\node[draw=none] (d1) at (1,-1) {$\cdots$};
\node[vertex] (sm) at (2,-1) [label=right:$S_m$]{}
 	edge[edge] node {} (v);
	
 \node[vertex] (x1) at (-1,-2) [label=left:$x_1$]{}
 	edge[edge] node {} (s1);

 \node[vertex] (x2) at (0,-2) [label=right:$x_2$]{}
   	edge[edge] node {} (s2)
 	edge[edge] node {} (s1);
 \node[draw=none] (d2) at (1,-2) {$\cdots$};
 \node[vertex] (xn) at (2,-2) [label=right:$x_n$]{}
  	edge[edge] node {} (s2)
 	edge[edge] node {} (sm);
	
\node[vertex] (u) at (0,-3) [label=below:$u$]{};

\draw[edge] (v) to (s1);
\draw[edge] (v) to (s2);
\draw[edge] (v) to (sm);
\draw[edge] (s1) to (v);
\draw[edge] (s2) to (v);
\draw[edge] (sm) to (v);
\draw[edge] (-2,-3) to (u);
\draw[edge] (-2,0) to (-2,-3);
\draw[edge] (v) to (-2,0);
\draw[edge] (u) to (x1);
\draw[edge] (u) to (x2);
\draw[edge] (u) to (xn);
\end{tikzpicture}
       
\caption{Multi-Signal Edge Max-Min instance of the set cover problem. For example lets say $S_1=\{x_1,x_2\}$, $S_2=\{x_2,x_n\}$, $S_m=\{x_n\}$}
\label{fig:np_hardness}
\end{figure}

Assume that every element $x_j$ is contained in exactly two subsets $S_{j_1}$ and $S_{j_2}$ (this is now the {\sc Vertex Cover} problem, an NP-hard special case of {\sc Set Cover}). The access from any node to any other node (with the exception of $x_j$ to $x_k$) is at least $\alpha^3$, since the shortest path connecting them has the length of at most $3$. Furthermore, for any $x_j$ and $x_k$, the there are exactly two paths ($x_j \rightarrow u \rightarrow v \rightarrow S_{k_1} / S_{k_2} \rightarrow x_k$) of length $4$ connecting them. Considering both paths, the access from $x_j$ to $x_k$ can be computed as $\alpha^2 (1 - (1 - \alpha^2)^2 )$, which is strictly less than $\alpha^3$ for $\alpha < \frac{\sqrt{5}-1}{2}$. Hence, for $\alpha < \frac{\sqrt{5}-1}{2}$ the minimum pairwise access in the graph is between any $x_j$ to any $x_k$ with value of $\alpha^2 (1 - (1 - \alpha^2)^2 )$.

We argue if there is a set cover, by adding the $k$ edges from $u$ to $S_i$ vertices corresponding to the set cover, we can increase the minimum pairwise access to at least $\alpha^3$. Note that now there is a path of length $3$ between any $x_j$ and $x_k \neq x_j$. Next, we show that if there is no set cover, then no matter how the $k$ edges are added, the minimum pairwise access over the graph would not increase and remain as $\alpha^2 (1 - (1 - \alpha^2)^2 )$ which is strictly less than $\alpha^3$. Hence, if there is a vertex cover, then the Multi-Signal Edge Max-Min solution would always return the $k$ edges from $u$ to vertices corresponding the vertex cover.

We prove by contradiction, assuming there is an edge set $E^+ = {e_1, e_2, ..., e_k}$ that will increase the minimum probability, while there is no vertex cover solution. As a consequence of lemma~\ref{} $E^+$ adds at least one additional path from any $x_j$ to any $x_k \neq x_j$. Now, we replace the edges in $E^+$ by another edge (or simply remove it if the new edge already exists), calling the set $E^'$ and argue that for each additional path connecting $x_j$ to $x_k$ using $E^+$, there is at least one alternative path (not equal to the first two paths) between them using $E^'$. According to lemma~\ref{}, $E^'$ is still increasing the minimum pairwise access of the graph (maybe not as much as $E^+$ but still increases the access compared to before the interventions). Now, we describe the edge replacement process, which takes place in $5$ stages.

\begin{itemize}
	\item Suppose there is an edge $e_i \in E^+$ from $z$ to $x_y$. We replace this edge with $z$ to $S_{y_1}$, and for every path $P_i$ connecting $x_j$ to $x_k$ that goes through $e_i = (z, x_y)$, we construct an alternative path using $e^'_i$ instead of $e_i$. Assume for each path $P_i$, $x_j$ goes through a path $P_{i,1}$ to $z$, then to $x_y$ using $e_i$, then through a path $P_{i,2}$ to $x_k$. Now we construct an alternative path, connecting $x_j$ to $x_k$ that is different than the two preciously existing paths. There are three possible cases: $(1)$ $S_{y_1}$ is contained in $P_1$: by taking part of $P_{i,1}$ $x_j$ can reach $S_{y_1}$, $S_{y_1}$ to $x_y$ using edges in $E$, and then through $P_{i,2}$ it reaches $x_k$. $(2)$ $S_{y_1}$ is contained in $P_2$: by taking $P_{i,1}$ $x_j$ can reach $z$, then to $S_{y_1}$ using $e^'_i$, then to $x_k$ through part of $P_{i,2}$. $(3)$ $S_{y_1}$ is not in the path: $x_j$ reaches $z$ through $P_{i,1}$, then to $S_{y_1}$ using $e^'_i$, then to $x_y$, and through $P_{i,2}$ to $x_k$.

	\item Suppose there is an edge $e_i \in E^+$ from $x_y$ to $z$. We replace this edge with $u$ to $z$. Using the same notations and process as above, there are three possible cases: $(1)$ $u$ is contained in $P_1$: $x_j$ through parts of $P_{i,1}$ can reach $u$ and through $e^'_i$ to $z$, then to $x_k$ through $P_{i,2}$. $(2)$ $u$ is contained in $P_2$: $x_j$ through $P_{i,1}$ can reach $x_y$ then to $u$ using edges in $E$, and then to $x_k$ through parts of $P_{i,2}$. $(3)$ $u$ is not in the path, $x_j$ to $x_y$ through $P_{i,1}$ then to $u$ and to $z$ using $e^'_i$, and then to $x_k$ through $P_{i,2}$.

	\item Suppose there is an edge $e_i \in E^+$ from $v$ to $u$. This edge is simply redundant since, for every path connecting $x_j$ to $x_k$, we can simply go through $x_j$ to $u$ using edges in $E$, and then taking $P_{i,2}$ to reach $x_k$.

	\item Suppose there is an edge $e_i \in E^+$ from $S_i$ to $u$. This edge is also redundant by considering three possible cases: $(1)$ any of the elements $x_i \in S_i$ is in $P_1$, then $x_j$ can reach $x_i$ through parts of $P_{i,1}$, then to $u$ using edges in $E$, then to $x_k$ through $P_{i,2}$. $(2)$ any element $x_i \in S_i$ is in $P_2$, then we go from $x_j$ to $S_i$ through $P_{i,1}$, then to $x_i$ using edges in $E$, then to $x_k$ through parts of $P_{i,2}$. $(3)$ no element $x_i \in S_i$ is in either $P_{i,1}$ or $P_{i,2}$, then using the same path, instead of going through $e_i = (S_i , u)$, we go from $S_i$ to any $x_i$ then to $u$ using edges in $E$.

	\item Suppose there is an edge $e_i \in E^+$ from $S_z$ to $S_i$, then we replace the edge with $u$ to $S_i$. There are two possible cases: $(1)$ $u$ is not contained in $P_2$:  $x_j$ can reach $u$ using edges in $E$, then to $S_j$ using $e^'_i$, then to $x_k$ through $P_{i,2}$. $(2)$ $u$ is contained in $P_2$: if there is an $x_z \neq x_j$ in $P_{i,1}$, then $x_j$ can reach $x_t$ through parts of $P_{i,1}$, then to $u$ using edges in $E$, and to $S_i$ using $e^'_i$ and through $P_{i,2}$ to $x_k$. Otherwise, $x_j$ can reach $S_z$ through - if there is any $x_z \in S_z$ in $P_{i,2}$, then to $x_z$ using edges in $E$ and taking parts of $P_{i,2}$ to $x_k$. Otherwise from $S_z$ to one of $x_z$, then to $u$ using the edges in $E$, and taking the rest of $P_{i,2}$ to $x_k$.

It is evident that these alternative paths can not be the same as the two previously existing paths. The new edge set $E^'$ contains only edges from $u$ to $S_i$, and these edges create at least one additional path from every $x_j$ to every $x_k \neq x_j$. Since we assumed there is no set cover, then there must exist an element $x_j$ that both sets containing it ($S_{j,1}$ and $S_{j,2}$) are not covered by edges from $u$. Then the access from any other element in $X$ to $x_j$ is still $\alpha^2 (1 - (1 - \alpha^2)^2 )$, and the minimum pairwise access has not changed. This is a contradiction since we assumed the minimum access has increased. This shows no matter which $k$ edges are added, we can not increase the minimum pairwise access if there is no set cover.

Now any algorithm that has an approximation ratio strictly better than $\frac{\alpha^2(1-(1-\alpha^2)^2)}{\alpha^3} = O(\alpha)$ must in fact be exact, and therefore also find the set cover. Even in the general case of {\sc Set Cover}, we can still distinguish between when there is and is not a set cover: The existence of a set cover still means the maximin probability is at least $\alpha^3$, while the lack of a set cover implies there is at least one vertex with probability no more than  $\alpha^2(1- (1- \alpha^2)^m)$, which is upper-bounded by $\alpha^3$ when $\alpha = 1/m$.  Therefore, since set cover is $O(\ln n)$-inapproximable, we cannot approximate the best $k$ edges to add without an additional $O(\ln n)$-factor edges.
\end{proof}

%This choice of representing function, may raise some questions. Is this function really chooses the poor nodes? In another way, can rich nodes have very low minimum access and be considered poor, or nodes with very low minimum access are the actual poor?

%In the experiment section, we compare the min reach node with the min absolute. If these nodes are almost the same, absolute may also be a good representation of reach in real-world networks.

%\svnote{I don't understand the point of this at all. I don't understand what you're trying to do in section 4.2. Specially I don't understand how the three propositions "prove" that absolute access doesn't allow "rich" nodes to be declared "poor". 1. Are you saying a) rich won't get richer if we intervene to improve the advantage of low-reach nodes? OR b)rich nodes have some specific structure that allows us to ignore them. 2. The "propositions" have "proofs". But there are not reasons. In here the "proof" is contained in the statement.}

%For further investigating this problem we make use of three assumptions:
%\begin{enumerate}
%	\item Rich nodes have high access to the majority: Any node can have high access to nodes close to it. But we define rich nodes as a node that have high access not only to its neighborhood but to a majority of nodes ($n/2 + 1$).
%	\item Choice of thresholds: We should set a threshold $t_h$ for high access. So if $p_{u,v} \geq t_h$, then nodes $u$ and $v$ have high access to each other. We select high and low thresholds in a way that low access threshold $t_l$ would not be greater than the square of the high access threshold ($t_l < t_h ^ 2$). This condition makes sense since it's basically saying that if a node have access to two other nodes, those nodes can't have low access to each other. This phenomenon is similar to forbidden triad in Granovetter's work which he argues that they are very unlikely to happen~\cite{granovetter77strength}.
%	\item There is at least one low access in the network.
%\end{enumerate}

%\svnote{Why is this a useful statement to prove? Who cares?}

%\begin{proposition}
%\Both ends of the access diameter can't be rich.
%\end{proposition}

%\begin{proof}
%Consider the case when both ends of the min access are rich. Since each one of them has high access to at least $n/2 + 1$ nodes, then there must be a node that have high access to both. Hence, they can't have low access to each other, so it is a contradiction since we assumed they have the minimum access to each other, and the minimum access is low.
%\end{proof}

%\begin{proposition}
%One end of the access diameter can be a rich node.
%\end{proposition}

%\begin{proof}
%Consider a clique of size over $n/2$ (all having complete access to each other), is connected to a path of length $p$. The maximum access distance is between the last node in the path and any rich node in the clique.
%\end{proof}

%\begin{proposition}
%Both ends of the access diameter can be "fairly" rich.
%\end{proposition}

%\begin{proof}
%Consider two cliques connected by a path of length k. Then again, the maximum access distance is between a node from the first clique and a node from the second clique.
%\end{proof}

%One argument against connecting poor nodes is that they're not active and we are wasting the budget on connecting them. One answer to this is that activity has correlation with influence. As a general rule, the more influence a person is, the more active she is. Poor nodes may not be active not because its in their nature, but because they don't have any voice/influence.

%\paragraph{Sanity Check}
%\begin{itemize}
%	\item Q: Is maximizing the minimum access actually connects the min nodes together? How? \\
%	A: Not always. Consider two paths of length 5, that both their middle nodes are connected to an 11th node \ref{fig:minmin_optima}. Here, the optimal intervention would be connecting $v_3$ to $v_9$ resulting min access of value $\alpha^5$, although our algorithm (connecting the mins) would connect one end of the first path (either $v_1$ or $v_5$) to another end of the second (either $v_7$ or $v_{11}$) resulting min access of value $\alpha^6 + \alpha^9 - \alpha^{11}$. \\

%	\item Q: Is the greedy algorithm optimal? If not, provide counterexamples. \\
%	A: Greedy solution is not always optimal. Consider the same example. For the second intervention, the greedy solution is not optimal cause the maximum min access it can reach is at most $\alpha^5 + 2*\alpha^6 - 2*\alpha^7 - \alpha^8 + \alpha^9$. Although our algorithm (connecting the mins) connects the two ends of first path to two ends of the second path, which is the optimal intervention resulting in min access of value $2*\alpha^5 + \alpha^6 + \alpha^8 - 2*\alpha^9 - 3*\alpha^{10} + 2*\alpha^{12}$. \\

%\begin{figure}
%\centering
%\tikzstyle{vertex}=[circle,fill=black,minimum size=5pt,inner sep=2pt]
%\tikzstyle{circled} = [draw, blue, thick, circle, minimum size=.55cm]
%\tikzstyle{edge}=[<-,color=black,line width=1.5]
%\tikzstyle{edgeback}=[->,color=black,line width=1.5]
%\tikzstyle{edgelabel}=[color=black]
%\begin{tikzpicture}[scale=0.8, auto]
     %draw the vertices and edges
	
%	\node[vertex] (s1) at (-3,-1) [label=below:$v1$]{};
%	\node[vertex] (s2) at (-1.5,-1) [label=below:$v2$]{}
%		edge[color=black,line width=1.5] node {} (s1);
%	\node[vertex] (s3) at (0,-1) [label=below:$v3$]{}
%		edge[color=black,line width=1.5] node {} (s2);
%	\node[vertex] (s4) at (1.5,-1) [label=below:$v4$]{}
%		edge[color=black,line width=1.5] node {} (s3);
%	\node[vertex] (s5) at (3,-1) [label=below:$v5$]{}
%		edge[color=black,line width=1.5] node {} (s4);
	
%	\node[vertex] (s11) at (-3,1) [label=above:$v7$]{};
%	\node[vertex] (s12) at (-1.5,1) [label=above:$v8$]{}
%		edge[color=black,line width=1.5] node {} (s11);
%	\node[vertex] (s13) at (0,1) [label=above:$v9$]{}
%		edge[color=black,line width=1.5] node {} (s12);
%	\node[vertex] (s14) at (1.5,1) [label=above:$v10$]{}
%		edge[color=black,line width=1.5] node {} (s13);
%	\node[vertex] (s15) at (3,1) [label=above:$v11$]{}
%		edge[color=black,line width=1.5] node {} (s14);
		
%	\node[vertex] (s) at (0,0) [label=left:$v6$]{}
%		edge[color=black,line width=1.5] node {} (s3)
%		edge[color=black,line width=1.5] node {} (s13);

%\end{tikzpicture}
%\caption{...}
%\label{fig:minmin_optimal}
%\end{figure}

%	\item Q: Can we have a situation with one vector (H, H, ..., H, L), and one (L+e, L+e, ...)? If yes, does this happen often? \\
%	A:
%	Assumption: Rich = have high access to majority of nodes
%	Assumption: $~$Transitive: (High $*$ High $>$ Low) -- if both nodes have high access to one other node, they don't have low access to each other (we can extend this to paths of length 3).
%	\begin{enumerate}
%		\item One end of the mins can be a rich node: consider a clique being connected to a path of length k. The algorithm connects one rich node of the clique to the poor node at the end of the path.
%		\item Although this is not a case that happens often in real-world networks. For this there should be a densely-connected part that only has one branch connected to it. If there are more than one branches, the algorithm would connected nodes on the branches.
%		\item Both ends can't be rich: For this there should be a node that both of the min ends have high access to. Hence, they can't have low access to each other. And since that was the minimum, there can't be a low access in the network.
%		\item Both nodes can be "fairly" rich. Consider two cliques connected to each other by a path of length k. The algorithm would connect one node from each clique to each other.
%		\item Again this case does rarely happens. Since after this intervention all of the rich nodes have (almost) high access to each other and they're not going to be chosen as the next mins.
%	\end{enumerate}

%\end{itemize}
